Price Manipulability in First-Price Auctions

First-price auctions have many desirable properties, including uniquely possessing some, like credibility. However, first-price auctions are also inherently non-truthful, and non-truthfulness may result in instability and inefficiencies. Given these pros and cons, we seek to quantify the extent to which first-price auctions are susceptible to manipulation. In this work we adopt a metric that was introduced in the context of bitcoin fee design markets: the percentage change in payment that can be achieved by being strategic. We study the behavior of this metric for single-unit and $k$-unit auction environments with $n$ i.i.d. buyers, and seek conditions under which the percentage change tends to zero as $n$ grows large. To the best of our knowledge, ours is the first rigorous study of the extent to which large multi-unit first price auctions are susceptible to manipulation. We provide an almost complete picture of the conditions under which they are truthful in the large, and exhibit some surprising boundaries.

==> abstract.tex <==
 First-price auctions have many desirable properties, including uniquely possessing some, like credibility. %\textcolor{teal}{A potential drawback of first-price auctions is that they are inherently non-truthful and agents may have an incentive to strategize.} 
 %In repeated settings bidders can learn how to bid over time, but this can render the system instable and lead to inefficiencies. It is thus central to understand, when and to which extent there is room for manipulation.  
 \textcolor{teal}{Their attractive properties have led to their adoption in ad exchanges for display ads.   However, first-price auctions are also inherently non-truthful, and non-truthfulness may result in instability and inefficiencies. In fact, empirical evidence from the early days of sponsored search showed that the by-then industry standard of using first-price auctions led to sawtooth bidding patterns. Given these pros and cons, we seek to quantify the extent to which first-price auctions are susceptible to manipulation.}
 
%For measuring proximity from truthfulness, 
\textcolor{teal}{In this work} we adopt a metric that was introduced in the context of bitcoin fee design markets: the percentage change in payment that can be achieved by being \textcolor{teal}{strategic}. \textcolor{teal}{We study the behavior of} this metric for single-unit and $k$-unit auction environments with $n$ i.i.d.~buyers, \textcolor{teal}{and seek conditions under which the percentage change tends to zero as $n$ grows large.}
%, where each buyer participates in the auction independently with probability $p$. 
For the single-unit case, we derive a sharp characterization of when the percentage change in payment goes to zero for any bounded-support distribution: if and only if \textcolor{teal}{$k = o(n)$}. 
For \textcolor{teal}{monotone hazard rate (MHR)} distributions, we show the same is true even for unbounded support distributions, and also show that MHR is necessary to be able to remove the bounded support restriction: for the class of  $\alpha$-strongly regular distributions for any $\alpha < 1$ \textcolor{teal}{($\alpha = 1$ is MHR)}, the boundedness is necessary to get percentage change in payment going to zero. For the $k$-unit case, we again derive a tight characterization: the percentage change in payment for any bounded-support distribution goes to zero if and only if \textcolor{teal}{$k = o(n)$}. \textcolor{teal}{We don't fully resolve the unbounded distribution case, but show that interestingly even for $k$ as small as $\sqrt{n}$ there are MHR distributions for which the price manipulability does \emph{not} vanish.}
\textcolor{teal}{All our results also extend to the case where participation in the auction is probabilistic, and bidders participate in the auction independently with probability $p$.}

\textcolor{teal}{To the best of our knowledge, ours is the first rigorous study of the extent to which large multi-unit first price auctions are susceptible to manipulation. We provide an almost complete picture of the conditions under which they are ``truthful in the large,'' and exhibit some surprising boundaries. An interesting avenue for future work, apart from settling the exact boundary for unbounded MHR distributions, is to examine the non-asymptotic behavior.}

==> intro.tex <==
\section{Introduction}\label{sec:intro}
First-price auctions enjoy many desirable properties including transparency (winners-pay-bid)  \textcolor{teal}{\cite[e.g.,][]{Krishna09}}, and uniquely possess some properties like credibility~\citep{AL20}. They have been put to use in a large variety of settings. Their attractive properties have been influential in causing the recent switch in the display ads industry's ad exchanges to first-price auctions. 
\textcolor{teal}{A potential drawback of first-price auctions is that they are not truthful. That is, bidders may benefit from misreporting their valuation/willingness to pay. Non-truthfulness is problematic for a number of reasons. A main concern is that in the absence of a dominant-strategy equilibrium, it's usually a non-trivial task to find an equilibrium bidding strategy. Moreover, if bidders have to learn how to bid then they will update their bids frequently, causing a lot of traffic to the website, and resulting in an instable and upredictable system as a whole.}

%% The paper is:
%% https://web.stanford.edu/~ost/papers/cycling.pdf

\textcolor{teal}{A cautionary tale regarding the use of first-price auctions comes from the early days of sponsored search \cite{Edelman07}. In their influential paper, Edelman and Ostrovsky performed an analysis of bidding data from Overture, which was one of the first companies to provide a paid placement service, and used a first-price auction to determine the allocation of ads and payments. Their analysis showed that bids were very unstable and often exhibited a sawtooth pattern of gradual price increases followed by sudden drops (cf.~Figure 2 in their paper).}

\textcolor{teal}{Given these pros and cons of first-price auctions, it seems indispensable---and of great practical relevance---to have tools that allow to quantify the extent to which first price-auctions are susceptible to manipulation, or put positively, how close to being incentive compatible they are.}

\subsection{Our Approach}

%%In this work we ask, \emph{exactly how truthful a first-price auction is}. 


%We study $k$-units first-price auctions for both $k=\Theta(1)$ and $k =o(n)$. The case of $k=\Theta(n)$ is trivial and can be easily shown to be susceptible to manipulation. We include it just for completeness. In a $k$-units first-price auctions, the highest $k$ bidders receive the good, and each of them pays their bid. The rest pay $0$. There are $n$ buyers, and their private values are drawn i.i.d. from some distribution with cdf $F$.

\textcolor{teal}{We adopt a notion of approximate incentive compatibility that  was recently introduced by \citep{LSZ19}, who used it to study different bitcoin fee designs.} The idea is to measure the maximum relative change in payment that any agent can achieve by being strategic. \textcolor{teal}{We use this metric to study the $k$-unit first-price auction with $n$ bidders, whose values are i.i.d.~draws from $F$. This auction receives one bid from each agent. The $k$ highest bidding agents ``win'' and are assigned one unit of the good, and have to pay their bid.}

\textcolor{teal}{To formally define the metric, for} any given valuation profile $\bv$, let $v_{(r)}$ denote the $r$-th largest value. 
%And let $\winners(\bv) = \{i | v_i \geq v_{(k)}\}$. 
Let $\ph_i(\bv) \equiv v_i$ whenever $v_i \geq v_{(k)}$ and $0$ otherwise, denote the agent $i$'s payment when all the agents, including $i$, bid their true value. Let $\ps_i(\bv) \equiv v_{(k+1)}$ whenever $v_i \geq v_{(k)}$ and $0$ otherwise, denote the smallest payment the agent $i$ can manage to get charged and still get allocated, when $i$ is strategic and all other agents are honest. The relative price change for agent $i$ is given by $\delta_i(\bv, n, k) \equiv 1 - \ps_i(\bv)/\ph_i(\bv)$ whenever $v_i \geq \bv_{(k)}$ and $0$ otherwise. The quantity of interest for us is 
\begin{align}\EE[\delta_{\max}(\bv, n, k)] \equiv \EE[\max_i \delta_i(\bv, n, k)] \textcolor{teal}{= 1 - \EE\left[\frac{\ps_i(\bv)}{\ph_i(\bv)}\right]},\label{eq:delta-max}
\end{align}
namely, the maximum relative price change that can occur for any agent. For brevity, from here on we drop the arguments of $\delta_{\max}$. 

In this work we ask the following: 
%\begin{enumerate}
%\item 
1) 
%When is a first-price auction almost truthful, i.e., when does $\EE[\delta_{\max}] \rightarrow$ 0? 
\johcomm{When do the benefits from bid manipulation vanish to zero in the large market limit, i.e., $\EE[\delta_{\max}] \rightarrow$ 0?}
%\item 
2) Which distributions allow $\EE[\delta_{\max}] \rightarrow 0$? 
%\item 
3) Do the distributions need to be bounded? Does regularity help? Does monotone hazard rate (MHR) help? 
%\end{enumerate}
The answers are not straightforward, and are \emph{not} as simple as letting $n \to \infty$ will automatically let $\EE[\delta_{\max}] \rightarrow 0$. 

\subsection{Discussion}

%\textcolor{teal}{[discuss metric: why is it desirable and different from other metrics?  (1) applicability no use of valuations (2) complete info (3) in all settings we consider asymptotically BNE = truthful, and in definitions above we could also ask for price manipuabilit with respect to equilibrium bids, we will see that BNE is not sufficient for no price manipuability  ]}

\textcolor{teal}{\noindent 1) \emph{Deviation from truthfulness or from BNE?} The definition in Equation~(\ref{eq:delta-max}) measures the maximum percentage price change \emph{assuming everyone else bids truthfully}. Wouldn't it be more natural to define it with respect to some Bayes-Nash equilibrium (BNE)? It turns out that for all settings we consider, that is whenever $k = o(n)$ and $n \rightarrow \infty$, then a) there is a unique BNE \cite{ChawlaH13} (this part is true for all $n$ and $k$) and b) a simple application of Myerson's payment identity \cite{Myerson81} shows that asymptotically the two quantities coincide.}

\medskip

\noindent\textcolor{teal}{2) \emph{Why this measure and not something else?} A first reason is that it's very practitioner friendly. Indeed, in sharp contrast to other metrics that have been proposed for measuring approximate incentive compatibility (see Section~\ref{sec:related}), the metric defined in Equation~(\ref{eq:delta-max}) does \emph{not} require the auctioneer to reverse engineer the agents' valuations to e.g.~draw conclusions about the utility they could gain from a misreport. It only requires knowledge of the bids and prices, which is precisely the data the auctioneer has access to. A second reason is that the notion of ICness captured by Equation~(\ref{eq:delta-max}) is ``ex post'' (or ``full info''). It measures the extent to which an agent that has learned about the other agents' bids can game the system.} 
%%
%A few desirable properties of this metric are: a) when it is close to zero, it is evidence that the auction is close to being truthful, b) when it is bounded away from zero, it is evidence\footnote{\johcomm{This is a quite common way of formalizing “truthfulness in the large”. For example, see definition 4 in \cite{Budish18} - they measure utility while we measure price changes, but other than that the concept of convergence to zero is the same.}} that there is room to manipulate/shade bids, and c)
%it is concrete and simple to compute: 
%\johcomm{it is concrete, simple to compute and does not need knowledge of true valuations:}
%if $X^n_{(r)}$ denotes the $r$-th order statistic among $n$ i.i.d. draws of a random variable, it follows that $\EE[\delta_{\max}(\bv,n,k)] = 1 - \EE\left[\frac{X^n_{(k+1)}}{X^n_{(1)}}\right]$.
\johcomm{As observed in \citep{Edelman07}{ (Section 4)}, there is indeed evidence that bidders observe their competitors' recent behavior and use this information to adjust their own bids.} 
%This justifies assuming complete information of all other bids. e) In this definition of the metric, any agent not winning the item is truthful. However, we later see that if these agents bid according to a BNE, asymptotically, the analysis remains the same. One conclusion is that the BNE assumption does not always suffice to guarantee no price manipulability.

\medskip

\noindent\textcolor{teal}{3) \emph{Expected ratio vs. ratio of expectations.}}
\johcomm{It is important to note that the main part of our analysis consists of studying the expectation of ratios of order statistics, which is non-trivial and quite different from the ratio of expectations of order statistics.} \textcolor{teal}{Indeed, if $X^n_{(r)}$ denotes the $r$-th order statistic among $n$ i.i.d. draws of a random variable, it follows that $\EE[\delta_{\max}(\bv,n,k)] = 1 - \EE\left[X^n_{(k+1)}/X^n_{(1)}\right].$}

\subsection{Our Results}

%\paragraph{Results and surprises} 
Our results are summarized in Table~\ref{tab:results_n}. The table is self-explanatory: for different classes of distributions, for different regimes of $k$ covering the whole spectrum from $k=1\dots n$, we ask whether every distribution in that class provides no room for bid manipulation (i.e., whether $\lim_{n\to\infty}\EE[\delta_{\max}] = 0$), or, whether there are distributions in that class permitting bid manipulation (i.e., whether $\lim_{n\to\infty}\EE[\delta_{\max}] > 0$). 

\begin{table}
  \caption{Relative price change for first-price auctions. The last rowis immediate, and has been included for completeness.}
  \label{tab:results_n}
  \centering
  \begin{tabular}{lllp{5cm}}
    \toprule
     & Bounded support & MHR, continuous &\parbox{5cm}{$\alpha$-strongly regular,\\  $\alpha \in [0,1)$}\\
    \midrule
    $k = \Theta(1)$  & $\lim_{n\to\infty}\EE[\delta_{\max}] = 0$  & $\lim_{n\to\infty}\EE[\delta_{\max}] = 0$  & $\lim_{n\to\infty}\EE[\delta_{\max}] > 0 $  \\
    $k = o(n)$      & $\lim_{n\to\infty}\EE[\delta_{\max}] = 0$ & $\lim_{n\to\infty}\EE[\delta_{\max}] > 0$  & $\lim_{n\to\infty}\EE[\delta_{\max}] > 0$\\
    \midrule
    $k = \Theta(n)$     & $\lim_{n\to\infty}\EE[\delta_{\max}] > 0$ & $\lim_{n\to\infty}\EE[\delta_{\max}] > 0$  & $\lim_{n\to\infty}\EE[\delta_{\max}] > 0$\\
    \bottomrule
  \end{tabular}
\end{table}

\textcolor{teal}{For the single-unit case, we derive a sharp characterization of when the percentage change in payment goes to zero for any bounded-support distribution: if and only if \textcolor{teal}{$k = o(n)$}. For \textcolor{teal}{monotone hazard rate (MHR)} distributions, we show the same is true even for unbounded support distributions, and also show that MHR is necessary to be able to remove the bounded support restriction: for the class of  $\alpha$-strongly regular distributions for any $\alpha < 1$ \textcolor{teal}{($\alpha = 1$ is MHR)}, the boundedness is necessary to get percentage change in payment going to zero. For the $k$-unit case, we again derive a tight characterization: the percentage change in payment for any bounded-support distribution goes to zero if and only if \textcolor{teal}{$k = o(n)$}. \textcolor{teal}{We don't fully resolve the unbounded distribution case, but show that interestingly for $k$ as small as $\sqrt{n}$ the price manipulability may \emph{not} vanish.}}

We remark on a few surprises and subtleties here. First, the class of MHR distributions\footnote{Intuitively MHR distributions are to be thought of as distributions with tails no heavier than the exponential distribution. See Section~\ref{sec:prelim} for a formal definition.} typically behave similarly, at least qualitatively, to the class of $\alpha$-strongly regular distributions\footnote{See Section~\ref{sec:prelim} for formal definitions of regular and $\alpha$-strongly regular distributions.}~\citep{CR14}. Note that MHR distributions are just $\alpha$-strongly regular distributions for $\alpha = 1$, and regular distributions are $\alpha$-strongly for $\alpha = 0$, with a whole spectrum of $\alpha \in (0,1)$ in between. Indeed, a similar question to ours was asked of a different mechanism: the guarded empirical revenue maximization algorithm (guarded ERM) in a recent NeurIPS'20 paper by~\cite{DLLQWY20}. They show that guarded ERM is incentive compatible as $n\to\infty$ for $\alpha$-strongly regular distributions for \emph{every} $\alpha > 0$. In stark contrast, in this paper, we establish a sharp separation between MHR ($1$-strongly regular) and $\alpha$-strongly regular distributions for every $\alpha < 1$, \emph{even for the $1$-unit auction, i.e., $k=1$}. We establish that MHR distributions have relative price change approaching $0$, while also producing an $\alpha$-regular distribution for every $\alpha<1$ where the relative price change doesn't vanish. Obtaining such a sharp separation entails finding the precise property that makes a distribution susceptible or robust to bid manipulation. We identify this quantity to be the limit of the ratio of the median-of-the-maximum-of-$n$-draws and median-of-the-maximum-of-$2n$-draws as $n\to\infty$. Roughly, we show that distributions where this ratio is strictly lesser than $1$ are susceptible to bid manipulation, while distributions where this ratio is $1$ (for not just $2n$ draws in the denominator, but $\ell n$ draws for any constant $\ell$), are robust to bid manipulation. The novelty is in arriving at this insight. \emph{The proofs are simple and clean to read after this key insight is found}.

Second, even within the class of MHR distributions, there is a reasonably sharp separation across different $k$. We show that for $k=\Theta(1)$, MHR distributions are robust to bid manipulation, but even for a reasonably small $k$ such as $k=\sqrt{n}$, MHR distributions provide room for bid manipulation. The technique again is to use the ratio of median metric described earlier. Whether MHR distributions are susceptible to manipulation for even smaller $k$ than $k=\sqrt{n}$ is an open question. 

\paragraph{Probabilistic participation.}

%\textcolor{teal}{[TODO: Reuse some of this in Sec 1.1, remove this section afterwards]}



%\johcomm{One may argue that bidding truthfully is known to be a dominated strategy in a first-price auction. Yet, we seek to investigate the benefits of bid manipulation when all but one bidder are truthful. One way of assessing this is to measure the ability of the bidder to influence the price they have to pay (which is just their bid, if they win, in the first-price auction) by shading their bids. In settings where the analysis shows that the price manipulability vanishes as $n$ goes to $\infty$, our claim is \emph{not} that bidders will switch to bidding truthfully. Rather, regardless of how they optimize their bids, the prices in the auction cannot be manipulated much. From an auctioneer's point-of-view, this is reassuring to hear. On the other hand, if the analysis shows that there is room for price manipulability, it is a useful caution to the auctioneer to mitigate the level of price manipulability by incorporating other tools like reserve prices in the auction.}\\

%\johcomm{Instead of asking whether truthfulness is an approximate equilibrium, it can also be of interest to study how close equilibrium is to truthfulness. That is, given a Bayesian Nash Equilibrium (BNE), perform an analysis that sheds light on how close the BNE is to truthfulness. We can use the same metric, and apply it to a BNE. In other words, when every other bidder except $i$ is bidding as in a BNE, how do the auction-clearing prices for $i$ compare when (a) $i$ bids truthfully versus (b) $i$ bids the highest BNE bid from other bidders (this is the absolute best bid $i$ can submit, even if $i$ has precise information about the highest other BNE bid), plus a vanishingly tiny $\epsilon$ just to be the highest, whenever $i$'s value exceeds the highest other BNE bid. In more detail, say for the single item case ($k=1$), instead of measuring the expectation of the ratio of the second highest value to the highest value (like we have done so far), we should now measure the expectation of the ratio of the second highest BNE bid to the highest value.}


%Here's our thinking: we completely agree with you that a first-price auction is not just non-truthful, but quite clearly so. This is because bidding truthfully is a dominated strategy in a first-price auction. Indeed, bidding anything lesser than their true value gives the bidder a positive (albeit often very tiny) expected utility, whereas bidding the true value gives zero utility. So bidding truthfully is certainly not a good default strategy. Our focus in this paper is not to ask whether a first-price auction becomes truthful in the large market limit. Instead we seek to investigate whether the benefits from bid manipulation vanish to zero in the large market limit, or if they are still bounded away from zero. One way of assessing this is to measure the ability of the bidder to influence the price they have to pay (which is just their bid, if they win, in the first-price auction) by shading their bids. Equivalently, it measures how susceptible to manipulation are the auction-clearing prices (i.e., transaction prices) in the large market limit. This is what we meant by "measuring proximity from truthfulness" in the abstract. We will make this clear in the next version of the paper. In settings where the analysis shows that the price manipulability vanishes as $n$ goes to $\infty$, our claim is *not* that bidders will switch to bidding truthfully. Rather, regardless of how they optimize their bids, the prices in the auction cannot be manipulated much. From an auctioneer's point-of-view, this is reassuring to hear. On the other hand, if the analysis shows that there is room for price manipulability, it is a useful caution to the auctioneer to mitigate the level of price manipulability by incorporating other tools like reserve prices in the auction.



%for every bounded support distribution (regardless of discrete/continuous/mixed), for \emph{any} value of $k = o(n)$ we have $\lim_{n\to\infty}\EE[\delta_{\max}] = 0$. Since $\EE[\delta_{\max}(\bv,n,k)] = 1 - \EE\left[\frac{X^n_{(k+1)}}{X^n_{(1)}}\right]$ (see preceding discussion), this immediately implies that $\lim_{n\to\infty} \EE\left[\frac{X^n_{(k+1)}}{X^n_{(1)}}\right]= 1$, even for very large values of $k$ such as $k = n^{1-\epsilon}$ and even $k = n/\log\log n$ say. I.e., even for such large values of $k$, the $k+1$-th order statistic among $n$ draws $X^n_{(k+1)}$ is asymptotically close to the first order statistic $X^n_{(1)}$. This is a counter-intuitive statement and it is further emphasized by the fact that it ceases to hold when we consider unbounded support distributions, even with the non-heavy-tailed restriction that MHR distributions come with. So our second point here is that there are MHR distributions for which $\lim_{n\to\infty}\EE[\delta_{\max}]  > 0$, i.e., $\lim_{n\to\infty} \EE\left[\frac{X^n_{(k+1)}}{X^n_{(1)}}\right]< 1$ even for reasonably small $k$ such as $k = \sqrt{n}$; contrastingly, we show that $\lim_{n\to\infty} \EE\left[\frac{X^n_{(k+1)}}{X^n_{(1)}}\right] = 1$ for $k = \Theta(1)$ for all continuous MHR distributions. Third, consider the interpolation between the class of regular distributions and MHR distributions using the class of $\alpha$-strongly regular distributions~\citep{CR14}. Regular distributions are at $\alpha = 0$ and MHR at $\alpha = 1$. We show that there are $\alpha$-strongly regular distributions for every value of $\alpha < 1$ s.t. $\lim_{n\to\infty}\EE[\delta_{\max}] > 0$. So our result for MHR distributions is quite sharp, and even distributions very close to MHR don't permit relative price change to vanish. We remark that a similar question was asked of the guarded empirical revenue maximization (guarded ERM) algorithm in a recent NeurIPS'20 paper by~\cite{DLLQWY20}, and they show that guarded ERM is incentive compatible as $n\to\infty$ for $\alpha$-strongly regular distributions for every $\alpha > 0$. And indeed, many other results that hold for MHR, continue to hold for $\alpha$-strongly regular distributions. In this backdrop, the fact that there is a sharp separation between MHR and $\alpha$-regular for every $\alpha < 1$ is surprising. In particular, the fact that first-price auctions have $\EE[\delta_{\max}] \to 0$ for $k=\Theta(1)$ and MHR is a surprise.

% \medskip

% \textcolor{teal}{[TODO: Where do we wnat to mention this?]}


%\paragraph{Probabilistic participation} 
All our results actually hold for a more general setting, namely, not all the $n$ agents need to participate. Each of the $n$ agents participates independently with a probability $p$. For $k=\Theta(1)$, for bounded support distributions, as long as $np = \omega(1)$ (a generalization of $n=\omega(1)$ for the simpler setting) all our results hold. For larger $k$, our results hold as long as $k = o(np)$ (a generalization of the $k=o(n)$ for the simpler setting). The probabilistic participation is practically motivated by quota-based throttling that happens in the display ads industry: many buyers cannot adequately handle the extremely high Queries-Per-Second (QPS) that an ad exchange sends them, and hence ask for the requests sent to them to be throttled. The latter is often done probabilistically. 
\subsection{Future Directions}

\textcolor{teal}{A first obvious open question is finding the exact boundary for (unbounded) MHR distributions with $k > 1$ units. We show that it may fail for $k \geq \sqrt{n}$ (so $k = o(n)$ is not sufficient), but how small does $k$ have to be?}


A \textcolor{teal}{second} general direction are feasibility constraints beyond $k$-units, such as matroids and beyond, along with probabilistic participation. A good place to start would be the $G(n,p)$ model where each edge in the graph participates independently with probability $p$. What can we show about the relative price change in these settings?

\textcolor{teal}{It would also be interesting to study the non-asymptotic behavior of the metric we proposed, e.g., in form of upper bounds on the percentage price change and how fast it decreases to zero as a function of $n, k$ and properties of the distribution.}

\subsection{Related work}\label{sec:related}

\paragraph{Relative price change metric}

The relative price change metric was introduced in the context of the bitcoin fee design market by~\cite{LSZ19}. The goal here was to analyze the monopolistic price (MP) mechanism. The MP mechanism solicits $n$ bids $b_1,\dots,b_n$ and sets a price $p$ that maximizes $k\cdot b_{(k)}$. To what extent is there a temptation for users to shade their bids in the MP mechanism was the question they studied. They showed that for finite support distributions, $\lim_{n \to \infty} \EE[\delta_{\max}] = 0$ for the MP mechanism, and conjectured that it should hold for all bounded support distributions. 
Later,~\cite{Yao20} confirmed the conjecture for all bounded support distributions in $[1,D]$, and also show that for regular distributions $\lim_{n \to \infty} \EE[\delta_{\max}] > 0$. More recently,~\cite{DLLQWY20} study the guarded\footnote{``Guarded'' just forces the monopolistic mechanism to pick a price that will let at least a certain minimum number of bids win} empirical revenue maximization mechanism, and show that even for $\alpha$-strongly regular distributions for any $\alpha > 0$, $\lim_{n \to \infty} \EE[\delta_{\max}] = 0$. 
In a different line of work,~\cite{Giannakopoulos21} consider anonymous posted price auctions for the setting of $n$ bidders with i.i.d values for one item. In order to obtain their results on MHR and strongly regular distributions, the authors also need to first establish statements involving tail bounds of order statistics. The technical challenges however differ from ours since they are concerned with the expectation of a single order statistic whereas we need to understand the fraction of the $k$-th over the largest order statistic.
To the best of our knowledge, we are the first to systematically study the first-price auctions with the same metric, and we cover the entire spectrum of $k$, and also $\alpha$'s in $\alpha$-strongly regular distribution. The results are reasonably different from those for the MP mechanism, including the separation between MHR and $\alpha$-strongly regular, the nuanced separation between $k=\Theta(1)$ and $k=\sqrt{n}$ even for MHR distributions etc.

\paragraph{Other approaches to approximate IC} \textcolor{teal}{There is a number of alternative approaches to measuring approximate incentive compatibility. A popular one is based on the notion of \emph{regret}, which measures how much an agent can improve her utility (= value minus payment) through a misreport. Different papers differ in how they aggregate regret across types and agents.}

\textcolor{teal}{Early examples that use a regret-based metric include \cite{ParkesKE01} and \cite{DayM08}. Both design approximately IC mechanisms by minimizing the distance to VCG payemnts. The former consider combinatorial exchanges and insist on IR and budget-balance and aim for approximate efficiency and approximate incentive compatibility. The latter design core-selecting combinatorial auctions that minimizes incentives for misreporting.}

\textcolor{teal}{Further examples include \cite{DuttingFJLLP12} and \cite{DuttingNPR19}. The former paper establishes a connection between the error in multi-class classification and expected ex-post regret, and shows how this enables fining maximally incentive payment rules for a given allocation rule through support vector machines. The other paper uses techniques from deep learning for finding revenue-maximizing auctions. It approximates IC through ex-post regret, which it approximates by sampling a few deviations and performing a couple of gradient descent steps.}

\textcolor{teal}{A number of papers, motivated by the difficulty of computing regret exactly, have proposed approaches for approximating it based on a number of samples \cite{BalcanSV19} or for approximating it computationally \cite {FengSS19,Colini-Baldeschi20}.}

\textcolor{teal}{A particularly relevant paper that uses a regret-based approach comes from \citet{AzevB18} who propose the concept of strategy-proofness in the large (SP-L). This notion requires that it is
approximately optimal for agents to report their types truthfully in sufficiently large markets.}

\textcolor{teal}{Another related line of work is on testing incentive compatibility \cite{LahaieEtAl18,DengL19}. Here the basic question is how agents participating in a repeated auction can test whether the auction is incentive compatible. Their approach is based on segmenting query traffic into buckets and systematically perturbing bids.}

\textcolor{teal}{A similar idea was used recently \cite{DengMLZ20} to propose a IC metric based on Myerson's payment identity. The notion compares the expected utility by uniform bid shading or bid inflation by a factor $(1+\alpha)$. It evaluates to $1$ if the auction is IC, if it is smaller or larger than that, then an agent may benefit from increasing/decreasing its bid uniformly.}

\textcolor{teal}{Other papers propose metrics of approximate IC that are applicable to settings where the utilities atre ordinal and doesn't involve money. \cite{PathakS13}, for example, proposes to rank mechanisms based on the number of instances that
are manipulable. Another direction is to define ``obvious manipulations'' and classify non-IC mechanisms into those that are obviously manipulable and those that are not \cite{TroyanM20}.}






% \textcolor{red}{TODO: Discuss related work on other ways to measure approx. IC (under construction)}

% \textcolor{teal}{A number of papers explore notions of regret to measure the degree to which a mechanism is incentive compatible. \citet{ParkesKE01} consider combinatorial exchanges and design rules that are approximately efficient and approximately truthful.}

% \textcolor{teal}{\citet{DuttingFJLLP12} show how structural support vector machines can be used to find payment rules for a given allocation rule with low expected ex-post regret. 
% \citet{DuttingNPR19} show how approximating incentive compatibility through the empirical ex-post regret enables the application of deep learning techniques for the design of revenue-maximizing mechanisms. They  approximate the maximum regret by sampling a few random deviations, and performing a limited number of gradient descent steps.  \citet{BalcanSV19} use tools from statistical learning to estimate the maximum ex-post regret.}

% \textcolor{teal}{\cite{DengLMZ20}}


